A Linear MPC with Control Barrier Functions for Differential Drive Robots

The need for fully autonomous mobile robots has surged over the past decade, with the imperative of ensuring safe navigation in a dynamic setting emerging as a primary challenge impeding advancements in this domain. In this paper, a Safety Critical Model Predictive Control based on Dynamic Feedback Linearization tailored to the application of differential drive robots with two wheels is proposed to generate control signals that result in obstacle-free paths. A barrier function introduces a safety constraint to the optimization problem of the Model Predictive Control (MPC) to prevent collisions. Due to the intrinsic nonlinearities of the differential drive robots, computational complexity while implementing a Nonlinear Model Predictive Control (NMPC) arises. To facilitate the real-time implementation of the optimization problem and to accommodate the underactuated nature of the robot, a combination of Linear Model Predictive Control (LMPC) and Dynamic Feedback Linearization (DFL) is proposed. The MPC problem is formulated on a linear equivalent model of the differential drive robot rendered by the DFL controller. The analysis of the closed-loop stability and recursive feasibility of the proposed control design is discussed. Numerical experiments illustrate the robustness and effectiveness of the proposed control synthesis in avoiding obstacles with respect to the benchmark of using Euclidean distance constraints. Keywords: Model Predictive Control, MPC, Autonomous Ground Vehicles, Nonlinearity, Dynamic Feedback Linearization, Optimal Control, Differential Robots.

==> docs/45329114-d11d-464c-8064-04de6ed5fe86 <==
{"id":"321241621323","lines":[{"id":"n0.3851416450923924","blocks":[],"style":{"align":"center"}},{"id":"n0.753572347805765","blocks":[{"id":"n0.5537664070045136","text":"\\diagram","type":"composite","elements":{"de8648182106231972":{"id":"de8648182106231972","lines":[{"id":"n0.15316515723192614","blocks":[{"id":"n0.8848186220232286","text":"y"}]}],"shape":{"data":{"p":{"x":377.8916111602609,"y":127.86958728937935},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de0108032002250813":{"id":"de0108032002250813","lines":[{"blocks":[{"id":"n0.9156795621424554","text":"x"}],"id":"n0.468730524027291"}],"shape":{"data":{"p":{"x":548.4499256528486,"y":227.14683747049273},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de8136810834072177":{"id":"de8136810834072177","lines":[{"id":"n0.862668785580589","blocks":[{"id":"n0.05889661649056266","text":"𝜃=u","style":{"color":[208,2,27,1]}},{"id":"n0.33260284726242073","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.3601983676714593","lines":[{"id":"n0.8118929596543227","blocks":[{"id":"n0.7999872883752117","text":"2"}]}]}},"style":{"color":[208,2,27,1]}}]}],"shape":{"data":{"p":{"x":506.6264859319947,"y":142.21672333697137},"rotation":0},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de3200999823458821":{"id":"de3200999823458821","lines":[{"blocks":[{"text":"x","id":"n0.7588107414151379"},{"id":"n0.01918564837799641","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5892298570493915","lines":[{"id":"n0.46824990486844076","blocks":[{"id":"n0.3084227231231329","text":"1"}]}]}}}],"id":"n0.8374545179356605"}],"shape":{"data":{"p":{"x":465.6094108472939,"y":217.84458547337059},"rotation":0},"anchor":"left-top","style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de887925277879686":{"id":"de887925277879686","lines":[{"blocks":[{"text":"x","id":"n0.8209670028739302"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.9294561567444823","text":"2"}],"id":"n0.930636641996551"}],"id":"n0.3834947987707138"}},"id":"n0.17168171515617314"}],"id":"n0.8685343449497589"}],"shape":{"data":{"p":{"x":394.6077595653117,"y":152.0401140620266},"rotation":0},"anchor":"left-top","style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de966714979712054":{"id":"de966714979712054","lines":[{"blocks":[{"text":"u","style":{"color":[208,2,27,1]},"id":"n0.4263176922131733"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.45900342014514384","text":"1"}],"id":"n0.6964118010891422"}],"id":"n0.8732082944731698"}},"style":{"color":[208,2,27,1]},"id":"n0.04061898254420315"},{"id":"n0.8692478527705423","text":"=V","style":{"color":[208,2,27,1]}}],"id":"n0.9928214072362058"}],"shape":{"data":{"p":{"x":433.9157121150664,"y":127.85350203592628},"rotation":0},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de6055515701510574":{"id":"de6055515701510574","lines":[{"id":"n0.12090665416472968","blocks":[{"id":"n0.8711929154674618","text":"y"},{"id":"n0.7126425823699891","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.22612094055209764","lines":[{"id":"n0.2771287902671633","blocks":[{"id":"n0.5961380221048911","text":"1"}]}]}}},{"text":"=x","id":"n0.045323902989375275"},{"id":"n0.050897629839753655","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.012025809105584484","lines":[{"id":"n0.4153209199462313","blocks":[{"id":"n0.8609098812647398","text":"1"}]}]}}}]}],"shape":{"data":{"p":{"x":604.0345458984375,"y":143.5730916547252},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de5992451288558609":{"id":"de5992451288558609","lines":[{"blocks":[{"text":"y","id":"n0.6888363865641896"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.35083444652896767","text":"2"}],"id":"n0.02290542786836447"}],"id":"n0.02254832764815462"}},"id":"n0.9948617941219495"},{"text":"=x","id":"n0.3560317856537729"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.2827941779968506","text":"2"}],"id":"n0.031277315659062443"}],"id":"n0.8285743883207932"}},"id":"n0.5281233949225419"}],"id":"n0.39465114151297476"}],"shape":{"data":{"p":{"x":602.8638833256091,"y":187.4061597244279},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de501965063294753":{"id":"de501965063294753","lines":[{"blocks":[{"id":"n0.31723232152599534","text":"x"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.4306013555303987","text":"req"}],"id":"n0.2257551473511512"}],"id":"n0.3667724543098212"}},"id":"n0.23188318008684483"}],"id":"n0.039919748509623876"}],"shape":{"data":{"p":{"x":9.490048116765978,"y":145.05854549887317},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de36892181972714666":{"id":"de36892181972714666","lines":[{"blocks":[{"id":"n0.37777962468757065","text":"y"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"req","id":"n0.12741087199138446"}],"id":"n0.36344215505269406"}],"id":"n0.12960617091917692"}},"id":"n0.9186528193135055"}],"id":"n0.19574277876332458"}],"shape":{"data":{"p":{"x":6.996592797212685,"y":200.13050849633953},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de17649389873998134":{"id":"de17649389873998134","lines":[{"id":"n0.0763736269024462","blocks":[{"id":"n0.7185331208155392","text":"𝛼"},{"id":"n0.5927609003568615","type":"single","text":"("},{"id":"n0.1292755938665413","text":"x"},{"id":"n0.6412249207087855","type":"single","text":")"},{"id":"n0.800113891458345","text":"+𝛽"},{"id":"n0.8227886510557436","type":"single","text":"("},{"id":"n0.8535599636713338","text":"x"},{"id":"n0.1778090451044152","type":"single","text":")"},{"id":"n0.7280469015348427","text":"v"}]}],"shape":{"data":{"p":{"x":158.45906928206904,"y":175.3342524472298},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de20285905148603756":{"id":"de20285905148603756","lines":[{"id":"n0.4810462400743709","blocks":[{"id":"n0.9078708726443341","text":"\\int","type":"composite","elements":{}}]}],"shape":{"data":{"p":{"x":290.44626216565143,"y":153.74766656681953},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de2577429662260011":{"id":"de2577429662260011","lines":[{"id":"n0.8231542886006395","blocks":[{"style":{"mathType":"\\mathcal"},"id":"n0.1272894368332309","text":"U"},{"id":"n0.8658691582889675","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.5751474456025283","lines":[{"id":"n0.8380218260535579","blocks":[{"id":"n0.7787442736959873","text":"2"}]}]}}},{"id":"n0.9163578912022796","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8558257433435397","lines":[{"id":"n0.5309561148418318","blocks":[]}]}}},{"id":"n0.40197081941971713","text":"=u"},{"id":"n0.42613523423431876","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.7749882374639783","lines":[{"id":"n0.4399284120999496","blocks":[{"id":"n0.5004985063563971","text":"2"}]}]}}}]}],"shape":{"data":{"p":{"x":273.7396364373676,"y":215.85791446097},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de5082873046099154":{"id":"de5082873046099154","lines":[{"blocks":[{"id":"n0.15503851055814755","text":"\\dot","type":"composite","elements":{"value":{"id":"n0.9795019934995153","lines":[{"id":"n0.09858700833262257","blocks":[{"id":"n0.9439600187918755","text":"𝜁"}]}]}}},{"text":"=","id":"n0.3140911285615473"},{"style":{"mathType":"\\mathcal"},"id":"n0.04388534488155904","text":"U"},{"id":"n0.4134323755434328","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.9697200614346522","lines":[{"id":"n0.5393107067669285","blocks":[{"id":"n0.7109835137079634","text":"1"}]}]}},"style":{}}],"id":"n0.8538416779299298"}],"shape":{"data":{"p":{"x":277.5929493015095,"y":125.98510262304114},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de29486381365880576":{"id":"de29486381365880576","lines":[{"blocks":[{"style":{"mathType":"\\mathcal"},"id":"n0.23134343384116818","text":"U"},{"id":"n0.7308112803027516","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8631040250998521","lines":[{"id":"n0.04320149725642608","blocks":[{"id":"n0.9030728559644845","text":"1"}]}]}},"style":{}}],"id":"n0.877177348729878"}],"shape":{"data":{"p":{"x":244.2923456420333,"y":151.1948355142834},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de7109683476396187":{"id":"de7109683476396187","lines":[{"blocks":[{"id":"n0.6254007343179446","text":"𝜁=u"},{"id":"n0.1385748868225749","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.975746618908292","lines":[{"id":"n0.43843387723788996","blocks":[{"id":"n0.14433137027793452","text":"1"}]}]}}}],"id":"n0.01453501467332341"}],"shape":{"data":{"p":{"x":319.339789956303,"y":149.88396358450427},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de5918429556846461":{"id":"de5918429556846461","lines":[{"blocks":[{"id":"n0.10831121555543843","text":"x"}],"id":"n0.8981554858878391"}],"shape":{"data":{"p":{"x":327.7050905389301,"y":329.8027590211826},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de06743802302824053":{"id":"de06743802302824053","lines":[{"id":"n0.8442010218876936","blocks":[{"id":"n0.5600981804495475","text":"DFL"}]}],"shape":{"data":{"p":{"x":185.32845190015888,"y":166.64047586538788},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de43314709809069063":{"id":"de43314709809069063","lines":[{"blocks":[{"id":"n0.6051599154120897","text":"unicycle Model"}],"id":"n0.38439382382999776"}],"shape":{"data":{"p":{"x":422.06292739462737,"y":243.3201812496633},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de8901794963399101":{"id":"de8901794963399101","lines":[{"blocks":[{"id":"n0.3463341297412261","text":"Extended Model of the unicycle"}],"id":"n0.12731664000564336"}],"shape":{"data":{"p":{"x":348.9829929157839,"y":71.7017456906129},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de22417982413644122":{"id":"de22417982413644122","lines":[{"blocks":[{"id":"n0.7288660596643641","text":"MPC"}],"id":"n0.35565278614624285"}],"shape":{"data":{"p":{"x":61.32845190015888,"y":180.64047586538788},"rotation":0},"anchor":"left-top"},"isTextMode":true},"de23809284718620383":{"id":"de23809284718620383","lines":[{"blocks":[{"text":"x","id":"n0.3574716840950958"}],"id":"n0.9666968304998727"}],"shape":{"data":{"p":{"x":60.70509053893011,"y":243.27999877929688},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de46851367440681946":{"id":"de46851367440681946","lines":[{"blocks":[{"text":"x","id":"n0.5903927134447704"}],"id":"n0.43145990689183944"}],"shape":{"data":{"p":{"x":189.7050905389301,"y":259.2799987792969},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de15151861987177284":{"id":"de15151861987177284","lines":[{"blocks":[{"id":"n0.6203007268348686","text":"v"},{"id":"n0.08869083473764072","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.025758374860507027","lines":[{"id":"n0.748840771427068","blocks":[{"id":"n0.8444582448630953","text":"1"}]}]}}}],"id":"n0.19134832228067777"}],"shape":{"data":{"p":{"x":130,"y":148.60831235641592},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de47284626398980567":{"id":"de47284626398980567","lines":[{"blocks":[{"text":"v","id":"n0.4782054527761199"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.7843769268860199","text":"2"}],"id":"n0.20193962080858063"}],"id":"n0.37453217739907196"}},"id":"n0.3398088754463455"}],"id":"n0.8598345446081441"}],"shape":{"data":{"p":{"x":131,"y":200.60831235641592},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de9952856543679676":{"id":"de9952856543679676","lines":[{"blocks":[{"text":"x","id":"n0.04942371214145158"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"req","id":"n0.48179801977672954"}],"id":"n0.6449230269558117"}],"id":"n0.5472870256451059"}},"id":"n0.2903010598045279"}],"id":"n0.5283562846968493"}],"shape":{"data":{"p":{"x":143,"y":114.05854549887317},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de8197166862153555":{"id":"de8197166862153555","lines":[{"blocks":[{"text":"y","id":"n0.7504708845486199"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"req","id":"n0.9585852921064704"}],"id":"n0.4253213550074084"}],"id":"n0.7348812993830489"}},"id":"n0.14704362750384048"}],"id":"n0.030756102128474794"}],"shape":{"data":{"p":{"x":173,"y":220.13050849633953},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true}},"connections":[],"intersections":{"id":"di9042511484984455","items":[],"style":{}},"shapes":[{"id":"dp6085234773052384","type":"axis2d","data":{"p1":{"x":380.489311606197,"y":129.63900999157127},"p2":{"x":545.5527194635677,"y":250.53663910101605},"cp":{"x":396.99565239193413,"y":238.44687619007158}}},{"id":"dp4039637339248099","type":"ellipse","data":{"p1":{"x":441.4581208592035,"y":149.90039286505862},"p2":{"x":491.1438453833531,"y":198.47123678380993}}},{"id":"dp0008367574813035183","type":"rectangle","data":{"p1":{"x":446.08437362727483,"y":165.90693779023297},"p2":{"x":468.7671797947861,"y":169.22772516782047},"skewX":-7.65,"rotation":311.43},"style":{"fillColor":[0,0,0,1]}},{"id":"dp824690192022622","type":"rectangle","data":{"p1":{"x":464.9924220664985,"y":181.7912978192112},"p2":{"x":487.6752282340096,"y":185.11208519679852},"rotation":311.43,"skewX":-7.65},"style":{"fillColor":[0,0,0,1]}},{"id":"da9341064531173986","data":[{"x":396.99565239193413,"y":238.44687619007158},{"x":506.9648655059687,"y":137.58119000606035}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da49694818891404635","data":[{"x":466.3009831212783,"y":174.18581482443426},{"x":565.2325249819432,"y":174.20346451731552}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da8474359741690485","data":[{"p1":{"x":491.9156024625051,"y":151.25938891990262},"cp":{"dx":7.624963710366785,"dy":0.03529938576252789},"cp2":{"dx":-2.3152712374559314,"dy":-12.79573446778798},"p2":{"x":522.7858856285843,"y":173.3210000712612}}],"head":"fh>","tail":"f<","shaft":"-","mVer":1,"type":"cubic","style":{"strokeColor":[65,117,5,1]}},{"id":"da2496465824438452","data":[{"x":465.6758617713378,"y":238.18213685625528},{"x":466.3009831212783,"y":174.18581482443426}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da031138574404262487","data":[{"x":397.7612388059635,"y":173.7622322942883},{"x":466.3009831212783,"y":174.18581482443426}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da6951548662744635","data":[{"x":466.3009831212783,"y":174.18581482443426},{"x":491.9156024625051,"y":151.25938891990262}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[208,2,27,1]}},{"id":"da6303486117265957","data":[{"x":476.33382515025403,"y":183.45169150800484},{"x":460.5128050276384,"y":168.8910281481082}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"dp15418933164525117","type":"rectangle","data":{"p1":{"x":369.50889216944324,"y":123.60378764541339},"p2":{"x":580.1605986710322,"y":259.82734062643317}}},{"id":"da1836305673690377","data":[{"x":578.7009567002119,"y":168.36788183001835},{"x":648.9956051262759,"y":168.43685735958326}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da6640695297319572","data":[{"x":579.3312612438606,"y":212.40775104333014},{"x":648.9956051262759,"y":213.26992542928596}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp1571891389187734","type":"rectangle","data":{"p1":{"x":159.760009765625,"y":152.0800018310547},"p2":{"x":246.76695294804492,"y":221.02949490288833}}},{"id":"da6848053056521872","data":[{"x":8.996592797212685,"y":174.2652769176649},{"x":34.760009765625,"y":174.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da817394865872092","data":[{"x":6.996592797212685,"y":202.13050849633953},{"x":36.45906928206904,"y":202.19948402590444}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da08523669735604167","data":[{"x":247.3972068729542,"y":172.67875375979742},{"x":283.2577997435958,"y":172.7477276448952}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp787084030325919","type":"rectangle","data":{"p1":{"x":284.28617005429027,"y":155.5042415702459},"p2":{"x":318.0899716848034,"y":193.43991455230207}}},{"id":"da6102027570975879","data":[{"x":320.57798396631824,"y":174.47207641680686},{"x":364.53286760641356,"y":174.47207806127398}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da12709295528607223","data":[{"x":247.59629037521654,"y":214.1320998152418},{"x":363.70353017924197,"y":214.13209817077464}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp8775953748528993","type":"rectangle","data":{"p1":{"x":269.98840090885,"y":90.84116262355931},"p2":{"x":603.3820466318373,"y":294.31431606466606}},"style":{"strokeType":"--"}},{"id":"da9815712491881761","data":[{"x":469.760009765625,"y":262.0800018310547},{"x":469.858720857208,"y":352.07999992370605}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da062107682622191795","data":[{"x":469.858720857208,"y":352.07999992370605},{"x":74.760009765625,"y":353.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da6605599981781962","data":[{"x":208.61743129815085,"y":351.21782553775023},{"x":207.78809387097925,"y":221.89166764437704}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da6005168394408558","data":[{"x":335.5554257863659,"y":174.4720772390404},{"x":336.760009765625,"y":50.08000183105469}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da20445038042343877","data":[{"x":336.760009765625,"y":50.08000183105469},{"x":195.760009765625,"y":49.08000183105469}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da7103118538202551","data":[{"x":195.760009765625,"y":49.08000183105469},{"x":196.760009765625,"y":132.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"dp30739963855387686","type":"rectangle","data":{"p1":{"x":37.760009765625,"y":152.0800018310547},"p2":{"x":124.76695294804495,"y":221.02949490288833}}},{"id":"da22138754801619953","data":[{"x":74.760009765625,"y":353.0800018310547},{"x":75.9306723384534,"y":220.7538439376815}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da4866197273999584","data":[{"x":125.99659279721268,"y":173.2652769176649},{"x":158.760009765625,"y":173.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da6197063620335217","data":[{"x":124.99659279721268,"y":199.2652769176649},{"x":157.760009765625,"y":199.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da22605940875548036","data":[{"x":6.996592797212685,"y":202.13050849633953},{"x":6.760009765625,"y":272.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da5597463936361262","data":[{"x":8.996592797212685,"y":174.2652769176649},{"x":8.760009765625,"y":88.08000183105469}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da4725221700175506","data":[{"x":8.760009765625,"y":88.08000183105469},{"x":172.760009765625,"y":89.08000183105469}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da9482378812237895","data":[{"x":172.760009765625,"y":89.08000183105469},{"x":172.760009765625,"y":151.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da6504442756591979","data":[{"x":6.760009765625,"y":272.0800018310547},{"x":170.760009765625,"y":273.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1},{"id":"da9617172636464295","data":[{"x":170.760009765625,"y":273.0800018310547},{"x":170.760009765625,"y":222.0800018310547}],"head":">","tail":"no","shaft":"-","mVer":1}],"settings":{"grid":false,"diagramHeight":377.2799987792969}}]},{"id":"n0.13244715860964873","blocks":[],"style":{"align":"center"}},{"id":"n0.6488787136616616","blocks":[{"id":"n0.9025973693512468","text":"\\diagram","type":"composite","elements":{},"connections":[],"intersections":{"id":"di4814839606457051","items":[],"style":{}},"shapes":[{"id":"dp9920535266245407","type":"ellipse","data":{"p1":{"x":283,"y":-282.3999938964844},"p2":{"x":406.760009765625,"y":-195.19998168945312}}},{"id":"dp26339108803950717","type":"rectangle","data":{"p1":{"x":71,"y":-335.3999938964844},"p2":{"x":627.760009765625,"y":-44.199981689453125}}}],"settings":{"grid":false,"diagramHeight":365.6071472167969}}]},{"id":"n0.9619378345448093","blocks":[],"style":{"align":"center"}},{"blocks":[],"id":"n0.3122327770809379"},{"id":"n0.45454348980757175","blocks":[{"id":"n0.40210480496042855","text":"\\diagram","type":"composite","elements":{},"connections":[],"intersections":{"id":"di07304218421291875","items":[],"style":{}},"shapes":[],"settings":{"grid":false,"gridBold":true,"diagramHeight":253.45455932617188}}]},{"id":"n0.25495317067195256","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"delayRenderCache":{"av":1310,"map":{}},"___version":2,"version":2,"av":1310}

==> docs/5a51ad6c-c0c7-4eea-9a4d-d7e489d0a620 <==
{"id":"r0.4359652835849005","lines":[{"id":"n0.40684905371754465","blocks":[]},{"id":"n0.13218580551042347","blocks":[{"id":"n0.5762222635848537","text":"\\diagram","type":"composite","elements":{"de21953577545469072":{"id":"de21953577545469072","lines":[{"blocks":[{"text":"y","id":"n0.7343651834886675"}],"id":"n0.6748863161366538"}],"shape":{"data":{"p":{"x":92.49522407103996,"y":75.94425966182335},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de25861177672350055":{"id":"de25861177672350055","lines":[{"blocks":[{"text":"x","id":"n0.8384960573484102"}],"id":"n0.6689855834127509"}],"shape":{"data":{"p":{"x":476.4641311124267,"y":295.5884084444584},"rotation":0},"anchor":"left-top"},"isMathDisplayMode":true},"de3195725883281424":{"id":"de3195725883281424","lines":[{"blocks":[{"text":"𝜃=u","style":{"color":[208,2,27,1]},"id":"n0.9826452500702461"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"2","id":"n0.021228488785787203"}],"id":"n0.9088797897595013"}],"id":"n0.8649507987693053"}},"style":{"color":[208,2,27,1]},"id":"n0.6840414451408892"}],"id":"n0.9739232872395269"}],"shape":{"data":{"p":{"x":406.0829291428089,"y":108.89875202815128},"rotation":0},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de2680489231810319":{"id":"de2680489231810319","lines":[{"blocks":[{"text":"x","id":"n0.206069812553608"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.26112521653601184"}],"id":"n0.7898099952048074"}],"id":"n0.11813754907030916"}},"id":"n0.1407066653408826"}],"id":"n0.3569746369741944"}],"shape":{"data":{"p":{"x":293.0977819531669,"y":276.22024182461234},"rotation":0},"anchor":"left-top","style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de12782337791641507":{"id":"de12782337791641507","lines":[{"blocks":[{"text":"x","id":"n0.29093413719479266"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"2","id":"n0.25395813509512744"}],"id":"n0.7682519996559622"}],"id":"n0.8772545332263768"}},"id":"n0.6939455397938961"}],"id":"n0.6778982087671714"}],"shape":{"data":{"p":{"x":133.2555220083364,"y":130.632334394985},"rotation":0},"anchor":"left-top","style":{"textColor":[208,2,27,1]}},"isMathDisplayMode":true},"de09854680165469265":{"id":"de09854680165469265","lines":[{"blocks":[{"text":"u","style":{"color":[208,2,27,1]},"id":"n0.9768547006130033"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.013724461051727088"}],"id":"n0.20138521376863605"}],"id":"n0.8812163852161679"}},"style":{"color":[208,2,27,1]},"id":"n0.1319663796107482"},{"text":"=V","style":{"color":[208,2,27,1]},"id":"n0.11116728544347354"}],"id":"n0.6707602245934796"}],"shape":{"data":{"p":{"x":243.64425916360562,"y":77.12110396991737},"rotation":0},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true}},"connections":[],"intersections":{"id":"di7399469973969535","items":[],"style":{}},"shapes":[{"id":"dp10527326326786168","type":"axis2d","data":{"p1":{"x":88.33331298828125,"y":66.52223659359095},"p2":{"x":459.9318275261089,"y":334},"cp":{"x":125.4931644420641,"y":307.2522236593591}}},{"id":"dp41012339815771903","type":"ellipse","data":{"p1":{"x":225.58916663655978,"y":111.34916508211612},"p2":{"x":337.4440087640377,"y":218.80884641621807}}},{"id":"dp3063738627248962","type":"rectangle","data":{"p1":{"x":236.25002868365758,"y":146.72461792153715},"p2":{"x":286.82258173073205,"y":154.14750707244568},"skewX":-6.67,"rotation":311.92},"style":{"fillColor":[0,0,0,1]}},{"id":"dp2156640373406007","type":"rectangle","data":{"p1":{"x":278.81671747331376,"y":181.86768172675895},"p2":{"x":329.3892705203877,"y":189.29057087766728},"rotation":311.92,"skewX":-6.67},"style":{"fillColor":[0,0,0,1]}},{"id":"da2823164691774209","data":[{"x":125.49316444206397,"y":307.2522236593591},{"x":373.06103407783144,"y":84.09376849620182}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da024845894972408855","data":[{"x":281.51658770029866,"y":165.0790057491671},{"x":504.2359321847306,"y":165.11805449157393}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da16194407987613113","data":[{"p1":{"x":339.1814246330032,"y":114.35585121736486},"cp":{"dx":17.16567726885586,"dy":0.07809748481363954},"cp2":{"dx":-5.212247606896597,"dy":-28.309690287539695},"p2":{"x":408.6780593916253,"y":163.16566205795056}}],"head":"fh>","tail":"f<","shaft":"-","mVer":1,"type":"cubic","style":{"strokeColor":[65,117,5,1]}},{"id":"da23078990924930687","data":[{"x":280.1092850881746,"y":306.66650592927215},{"x":281.51658770029866,"y":165.0790057491671}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da36824992864705486","data":[{"x":127.21668861920614,"y":164.14185827476211},{"x":281.51658770029866,"y":165.0790057491671}],"head":"no","tail":"no","shaft":".","mVer":1},{"id":"da9512001978314766","data":[{"x":281.51658770029866,"y":165.0790057491671},{"x":339.1814246330032,"y":114.35585121736486}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[208,2,27,1]}},{"id":"da9697384040426567","data":[{"x":304.10299399685084,"y":185.57912630221304},{"x":268.4859686830569,"y":153.3646511474265}],"head":"no","tail":"no","shaft":".","mVer":1}],"settings":{"grid":false,"diagramHeight":348}}]},{"id":"n0.4821695487499229","blocks":[],"style":null},{"id":"n0.20990238935081562","blocks":[]},{"id":"n0.049449145414143025","blocks":[]},{"id":"n0.8059811039567859","blocks":[]},{"id":"n0.03349021350930648","blocks":[],"style":null},{"id":"n0.23484221516954817","blocks":[],"style":null},{"id":"n0.35231590876365204","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":510,"delayRenderCache":{"av":510,"map":{}}}

==> docs/711e39a6-3145-49cc-8c0e-e79541a5432c <==
{"id":"r0.34160594011228596","lines":[{"id":"n0.2938207061685979","blocks":[]},{"id":"n0.6477179980581158","blocks":[{"id":"n0.8241367707399463","text":"\\diagram","type":"composite","elements":{"de47666471259340915":{"id":"de47666471259340915","lines":[{"id":"n0.9881458297804255","blocks":[{"id":"n0.035406368625289675","text":"predefined path"}]}],"shape":{"data":{"p":{"x":254.7652993876614,"y":110.67974923658969}},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[65,117,5,1]}},"isTextMode":true},"de9150741619326592":{"id":"de9150741619326592","lines":[{"blocks":[{"text":"Obsctale free path","id":"n0.4861746672809921"}],"id":"n0.20696762398708923"}],"shape":{"data":{"p":{"x":120.7652993876614,"y":214.6797492365897}},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[65,117,5,1]}},"isTextMode":true},"de2317201505374984":{"id":"de2317201505374984","lines":[{"id":"n0.1395983081973966","blocks":[{"id":"n0.2581747362892295","text":"e"},{"id":"n0.21797352278194326","text":"\\index","type":"composite","elements":{"indexValue":{"id":"n0.8891312123572068","lines":[{"id":"n0.3982797496260402","blocks":[{"id":"n0.6905642492300201","text":"B1"}]}]}}}]}],"shape":{"data":{"p":{"x":3,"y":18}},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de3038475738096611":{"id":"de3038475738096611","lines":[{"blocks":[{"text":"e","id":"n0.8798443381426151"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"B2","id":"n0.10337045220296148"}],"id":"n0.27519969515785814"}],"id":"n0.9052124897592628"}},"id":"n0.18971707954225447"}],"id":"n0.302308632425188"}],"shape":{"data":{"p":{"x":106,"y":6}},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de6138708054635691":{"id":"de6138708054635691","lines":[{"blocks":[{"text":"e","id":"n0.5916405006211336"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"text":"1","id":"n0.14557744518557958"}],"id":"n0.6268046892349657"}],"id":"n0.045284456874158385"}},"id":"n0.5708655187744622"}],"id":"n0.5144825609838639"}],"shape":{"data":{"p":{"x":94,"y":114}},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de5655153268552147":{"id":"de5655153268552147","lines":[{"blocks":[{"text":"e","id":"n0.394070380253809"},{"text":"\\index","type":"composite","elements":{"indexValue":{"lines":[{"blocks":[{"id":"n0.6572773097214488","text":"2"}],"id":"n0.07053478911458799"}],"id":"n0.5280536459821217"}},"id":"n0.7561109226066967"}],"id":"n0.20423836317981192"}],"shape":{"data":{"p":{"x":212.33331298828125,"y":93}},"anchor":"left-top","style":{"textColor":[65,117,5,1]}},"isMathDisplayMode":true},"de9213671511789758":{"id":"de9213671511789758","lines":[{"blocks":[{"id":"n0.4950617344067074","text":"Obsctale"}],"id":"n0.5838784467704701"}],"shape":{"data":{"p":{"x":378.7652993876614,"y":165.67974923658969}},"anchor":"left-top","settings":{"fontSize":"\\normalsize"},"style":{"textColor":[0,0,0,1]}},"isTextMode":true},"de046376429204134206":{"id":"de046376429204134206","lines":[{"blocks":[{"id":"n0.3831400760818744","text":"Target Point"}],"id":"n0.1716185827470813"}],"shape":{"data":{"p":{"x":566.7652993876613,"y":169.67974923658969}},"anchor":"left-top","settings":{"fontSize":"\\small"},"style":{"textColor":[65,117,5,1]}},"isTextMode":true}},"connections":[],"intersections":{"id":"di9219655300299334","items":[],"style":{}},"shapes":[{"id":"dp42405605052298645","type":"image","data":{"p1":{"x":113.89467548665817,"y":65.70672112416872},"p2":{"x":197.656833846187,"y":136.6213648746044},"url":"data-resources/7fb6da03-70d1-4e1a-bd29-178938e911ac","rotation":358.58}},{"id":"dp7131734775619587","type":"flow-magnetic-disk","data":{"p1":{"x":362,"y":103},"p2":{"x":461.33331298828125,"y":229}},"style":{"fillColor":[155,155,155,1]}},{"id":"da29450260892986857","data":[{"x":57.833343505859375,"y":14.5},{"x":111.33331298828125,"y":37}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[208,2,27,1],"thickness":2}},{"id":"da023838954287926484","data":[{"x":57.833343505859375,"y":14.5},{"x":23.166656494140625,"y":46.5}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[208,2,27,1],"thickness":2}},{"id":"da31458926460126624","data":[{"x":158,"y":97},{"x":226.33331298828125,"y":123}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[208,2,27,1],"thickness":2}},{"id":"da6099574324999388","data":[{"x":158,"y":97},{"x":108.33331298828125,"y":141}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"strokeColor":[208,2,27,1],"thickness":2}},{"id":"da10350356721829601","data":[{"p1":{"x":158,"y":97},"p2":{"x":609.3333129882812,"y":225},"cp":{"dx":56.33331298828125,"dy":64},"cp2":{"dx":-49,"dy":32}}],"head":"no","tail":"no","shaft":".","mVer":1,"type":"cubic","style":{"thickness":2}},{"id":"da6970642554735229","data":[{"x":293,"y":166},{"x":292.33331298828125,"y":131}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[65,117,5,1],"strokeColor":[65,117,5,1]}},{"id":"da8572172325272911","data":[{"p1":{"x":158,"y":97},"p2":{"x":609.3333129882812,"y":225},"cp":{"dx":-29.66668701171875,"dy":111},"cp2":{"dx":-87,"dy":76}}],"head":"no","tail":"no","shaft":"-","mVer":1,"type":"cubic"},{"id":"da7088558211607838","data":[{"x":226.33331298828125,"y":188},{"x":200.33331298828125,"y":214}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[65,117,5,1],"strokeColor":[65,117,5,1]}},{"id":"dp9482744310861109","type":"ellipse","data":{"p1":{"x":602.3333129882812,"y":217.5},"p2":{"x":616.3333129882812,"y":232.5}},"style":{"strokeColor":[208,2,27,1],"thickness":2}},{"id":"da0863371705196152","data":[{"x":609.3333129882812,"y":225},{"x":608.6666259765625,"y":190}],"head":">","tail":"no","shaft":"-","mVer":1,"style":{"fillColor":[65,117,5,1],"strokeColor":[65,117,5,1]}}],"settings":{"grid":false,"diagramHeight":258}}]},{"id":"n0.1584022149661246","blocks":[],"style":null}],"pageSettings":{"pageSize":{"width":700}},"___version":2,"version":2,"av":448,"delayRenderCache":{"av":448,"map":{}}}
